PathoJev: Efficient Pathology Decisions from Shared Visual Context

Pathology workflows require multiple visual judgments about the same slide, from identifying tumor type to assessing grade and invasion. Generating and parsing a separate textual response for each structured question adds latency between visual evidence and usable decisions. Building on the System One paradigm, we introduce PathoJev, a pathology model that directly predicts answer probabilities for whole-slide and region-level assessment. PathoJev encodes each slide once and evaluates independent question suffixes in batches over the shared visual context. Reusing the hybrid backbone's recurrent states further limits the computation that grows with slide-context length for each additional question. Across three whole-slide benchmarks, the 9B and 27B models achieve mean accuracies of 77.2% and 78.1%, exceeding SlideChat by 5.4 and 6.3 percentage points. Both scales also maintain competitive accuracy on five ROI benchmarks. On WSI-Bench, the 9B model runs 9.1x faster than SlideChat. Shared context accelerates eight-question workloads by 6.9x and 5.9x over separate prefix encoding, rising to 11.2x and 8.9x for 64 questions. These results provide a reusable probabilistic interface for combining multiple visual judgments in whole-slide and local tissue assessment. Code: https://github.com/ChyaZhang/PathoJev.

==> sec/llm_usage.tex <==
\section*{LLM Usage Statement}
\textit{To be completed before submission.}

% Draft retained for final author review:
% OpenAI ChatGPT/Codex assisted with manuscript drafting and revision, literature lookup, LaTeX preparation, and plotting code. Anthropic Claude assisted with an initial manuscript review and revision planning. The tools produced draft text, code, and suggestions for author review. Qwen3.5-9B was used to decompose pathology report summaries into atomic statements, generate perturbed statements, and assign entailment-based silver labels for CF-Path.

